VertAttack: Taking advantage of Text Classifiers' horizontal vision

Text classification systems have continuously improved in performance over the years. However, nearly all current SOTA classifiers have a similar shortcoming, they process text in a horizontal manner. Vertically written words will not be recognized by a classifier. In contrast, humans are easily able to recognize and read words written both horizontally and vertically. Hence, a human adversary could write problematic words vertically and the meaning would still be preserved to other humans. We simulate such an attack, VertAttack. VertAttack identifies which words a classifier is reliant on and then rewrites those words vertically. We find that VertAttack is able to greatly drop the accuracy of 4 different transformer models on 5 datasets. For example, on the SST2 dataset, VertAttack is able to drop RoBERTa's accuracy from 94 to 13%. Furthermore, since VertAttack does not replace the word, meaning is easily preserved. We verify this via a human study and find that crowdworkers are able to correctly label 77% perturbed texts perturbed, compared to 81% of the original texts. We believe VertAttack offers a look into how humans might circumvent classifiers in the future and thus inspire a look into more robust algorithms.

==> defense.tex <==
\section{Exploratory Defenses}
Here we examine a few ways classifiers might defend themselves in order to combat \textit{VertAttack}. First, we examine if preprocessing is able to defend through back stepping. Second, we examine if adversarial training on the vertical text helps the classifier. 

\noindent \textbf{Preprocessing:}
...

\noindent \textbf{Adversarial training:}
The trickiness of \textit{VertAttack} is that the words do not change, but their presentation does. Thus, if classifiers could recognize words vertically, then they would have less trouble against this type of attack. Hence, we see if training on the vertical data allows the classifier to recognize and classifier the words better. 
Specifically, for the model we use a BERT classifier fine-tuned on a combination of the original training data and an equal portion of \textit{VertAttack} augmented data. That is we use x of the training data and apply \textit{VertAttack} to that same x training data, resulting in 2 * x training examples. 


==> nlg.tex <==
\section{\textit{VertAttack} with NLG}
The downside of the base version of \textit{VertAttack} (as well as other SOTA attacks) is that the algorithm must first search for the correct words to replace. This searching can result in a high number of queries. If an attack algorithm is querying an online classifier (or website), then these high number of queries could give away that attack. 
%we apply nlg to combine the steps ...
To improve this, we conduct preliminary experiments leveraging natural language generation models to combine both the selection and modification step. 
%

\noindent \textbf{Model and experiments:}
We fine-tune a pretrained BART model \cite{lewis2019bart} for this task. For fine-tuning we use 900 of the 1000 samples augmented by the base \textit{VertAttack} algorithm. This leaves 100 samples for testing purposes. 
%
We specifically use the data from the highest overall performing model (... Section \ref{}). 
%
Our training of the BART model is performed on ... gpus... took x hours...
%
We test on all previously noted datasets (Section \ref{}). 

\noindent \textbf{NLG Attack Results:} Table \ref{} show the overall results for the NLG model. We find that ...




